Bayesian Optimization for Iterative Learning

The performance of deep (reinforcement) learning systems crucially depends on the choice of hyperparameters. Their tuning is notoriously expensive, typically requiring an iterative training process to run for numerous steps to convergence. Traditional tuning algorithms only consider the final performance of hyperparameters acquired after many expensive iterations and ignore intermediate information from earlier training steps. In this paper, we present a Bayesian optimization (BO) approach which exploits the iterative structure of learning algorithms for efficient hyperparameter tuning. We propose to learn an evaluation function compressing learning progress at any stage of the training process into a single numeric score according to both training success and stability. Our BO framework is then balancing the benefit of assessing a hyperparameter setting over additional training steps against their computation cost. We further increase model efficiency by selectively including scores from different training steps for any evaluated hyperparameter set. We demonstrate the efficiency of our algorithm by tuning hyperparameters for the training of deep reinforcement learning agents and convolutional neural networks. Our algorithm outperforms all existing baselines in identifying optimal hyperparameters in minimal time.

==> Framework_v2.tex <==

\paragraph{Problem setting.}

We consider training a machine learning algorithm given a $d$-dimensional
hyperparameter $\bx\in\mathcal{X}\subset\mathcal{R}^{d}$ for $t$
iterations. This process has a training time cost $c(\bx,t)$ and
produces training evaluations $r(\cdot\mid\bx,t)$ for $t$ iterations, $t\in[T_{\min},T_{\max}]$.
 These could be episode rewards in DRL or training accuracies in DL.
An important property of iterative training is that we know the whole
curve at preceding steps $r(t' \mid \bx,t),$ $\forall t'\le t$.  

Given the raw training curve $r(\cdot\mid \bx,t)$, we assume an underlying
smoothed black-box function $f$, defined in Sec. \ref{subsec:Training-curve-compression}.
Formally, we aim to find $\bx^{*}=\arg\max_{\bx\in X}f(\bx,T_{\textrm{max}})$;
at the same time, we want to keep the overall training time, $\sum_{i=1}^{N}c(\bx_{i},t_{i})$,
of evaluated settings $[\bx_i, t_i]$ as low as possible. We summarize
our variables in Table $1$ in the supplement for ease of reading.


\subsection{Selecting a next point using iteration-efficient modeling \label{subsec:joint_modeling}}

We follow the popular designs in \cite{Krause_2011Contextual,Swersky_2013Multi,klein2017fast,song2019general}
to model the black-box function $f(\bx,t)$ and the cost $c(\bx,t)$
using two independent GPs. Each GP is designed to capture the correlation
across hyperparameter $\bx$ and iteration $t$ as follows\vspace{-12pt}

\begin{minipage}[t]{0.48\columnwidth}%
\begin{align*}
f(\bx,t) & \sim GP\left(0,K([\bx,t],[\bx',t'])\right)
\end{align*}
%
\end{minipage}%
\begin{minipage}[t]{0.48\columnwidth}%
\begin{align*}
c(\bx,t) & \sim GP(0,K_{c}([\bx,t],[\bx',t']))
\end{align*}
%
\end{minipage}

where $[\bx,t]\in\mathcal{R}^{d+1}$; $K$ and $K_{c}$ are the respective
covariance functions. In both models, we choose the covariance kernel
as a product $k\left([\bx,t],[\bx',t']\right)=k(\bx,\bx')\times k(t,t')$
 to induce similarities over parameter and iteration space. 
We estimate the predictive mean and uncertainty of both GPs at any
input $\bz_{*}=[\bx_{*},t_{*}]$ as\vspace{-15pt}

\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\mu\left(\bz_{*}\right)= & \mathbf{k}_{*}\left[\mathbf{K}+\sigma_{y}^{2}\idenmat\right]^{-1}\mathbf{y}\label{eq:mu_f}\\
\sigma^{2}\left(\bz_{*}\right)= & k_{**}-\mathbf{k}_{*}\left[\mathbf{K}+\sigma_{y}^{2}\idenmat\right]^{-1}\mathbf{k}_{*}^{T}\label{eq:sigma_f}
\end{align}
%
\end{minipage}%
\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\mu_{c}\left(\bz_{*}\right)= & \mathbf{k}_{c*}\left[\mathbf{K}_{c}+\sigma_{c}^{2}\idenmat\right]^{-1}\mathbf{c}\label{eq:mu_c}\\
\sigma_{c}^{2}\left(\bz_{*}\right)= & k_{**}-\mathbf{k}_{c*}\left[\mathbf{K}_{c}+\sigma_{c}^{2}\idenmat\right]^{-1}\mathbf{k}_{c*}^{T}
\end{align}
%
\end{minipage}

\hspace{-2pt}where $\mathbf{c}=[c_{i}]_{\forall i}$, $\by=[y_{i}]_{\forall i}$,
$\ensuremath{\bk_{*}=[k\left(\bz_{*},\bz_{i}\right)]_{\forall i}}$,
$\ensuremath{\mathbf{K}=\left[k\left(\bz_{i},\bz_{j}\right)\right]_{\forall i,j}}$,
$\ensuremath{k_{**}=k\left(\bz_{*},\bz_{*}\right)}$, $\ensuremath{\bk_{c*}=[k_{c}\left(\bz_{*},\bz_{i}\right)]_{\forall i}}$,
$\ensuremath{\mathbf{K}_{c}=\left[k_{c}\left(\bz_{i},\bz_{j}\right)\right]_{\forall i,j}}$,
$\sigma_{y}^{2}$ is the noise variance for $f$ and $\sigma_{c}^{2}$
is the noise variance for cost. We only require the predictive mean
of the cost function $\mu_{c}$ for the construction of our acquisition
function in Eq. (\ref{eq:querying_new_point}) since the uncertainty
of the cost $\sigma_{c}^{2}$ is less important. We maintain and optimize
the kernel hyperparameters (such as length-scale and noise variance)
of $K_{c}$ independently from $K$.

\begin{figure}
    \includegraphics[width=0.72\columnwidth]{fig/illustration_2d_reward}\includegraphics[width=0.27\textwidth]{fig/preference_function/merge_three_plots.pdf}
\centering{}\caption{Left:  the score in pink box is a convolution of the reward curve $r(\cdot\mid \bx =0.9, t=500)$ and a Sigmoid function $l(u \mid g_0, m_0 )=\frac{1}{1+\exp\left(-g_{0}\left[u-m_{0}\right]\right)}$
up to this time step. Bottom: observations are selected to augment
the dataset (red dots). The heatmap indicates the GP predictive mean
$\mu$ for $f$ across number of episode $t$ used to train an agent.
$T_{\min}$ and $T_{\max}$ are two user-defined thresholds of number
of used episodes for training. $x$ is a hyperparameter to be tuned.
Right: we learn the optimal parameter $g_{0}^{*}$ and $m_{0}^{*}$
for each experiment respectively.\label{fig:VirtualObs_LogisticScore-3}}
\vspace{-10pt}
\end{figure}

Our intuition is to select a point with high function value (exploitation),
high uncertainty (exploration) and low cost (cheap). At each iteration
$n$, we query the input parameter $\bx_{n}$ and the number of iteration
$t_{n}$ \cite{Snoek_2012Practical,wu2019practical}: 
\begin{align}
\bz_{n}=[\bx_{n},t_{n}] & =\underset{\bx\in\mathcal{X},t\in[T_{\min},T_{\max}]}{\arg\max}\alpha(\bx,t)/\mu_{c}(\bx,t).\label{eq:querying_new_point}
\end{align}
Although our framework is  available for any acquisition
choices \cite{Hernandez_2014Predictive,Wu_NIPS2016Parallel,letham2019constrained},
to cope with output noise, we follow \cite{Wang_2014Theoretical}
to use a slight modification of the incumbent as $\mu_{n}^{\max}$
which is the maximum of GP mean. Let $\lambda=\frac{\mu_{n}\left(\bz\right)-\mu_{n}^{\textrm{max}}}{\sigma_{n}\left(\bz\right)}$,
we then have a closed-form for the expected improvement (EI) as $\alpha_{n}^{\textrm{EI}}\left(\bz\right)=\,\sigma_{n}\left(\bz\right)\phi\left(\lambda\right)+\left[\mu_{n}\left(\bz\right)-\mu_{n}^{\textrm{max}}\right]\Phi\left(\lambda\right)$
where $\phi$ is the standard normal p.d.f., $\Phi$ is the c.d.f,
$\mu_{n}$ and $\sigma_{n}$ are the GP predictive mean and variance
defined in Eq. (\ref{eq:mu_f}) and Eq. (\ref{eq:sigma_f}), respectively.


\subsection{Training curve compression and estimating the transformation function\label{subsec:Training-curve-compression}}


Existing BO approaches \cite{chen2018bayesian,li2018hyperband} typically
define the objective function as an average loss over the final learning
episodes. However, this does not take into consideration how stable
performance is or the training stage at which it has been achieved.
We argue that averaging learning losses is likely misleading due to
the noise and fluctuations of our observations (learning curves) --
particularly during the early stages of training. We propose to compress
the whole learning curve into a numeric score via a preference function
 representing the user's desired training curve. In the following,
we use the Sigmoid function (specifically the Logistic function) to
compute the utility score as
\begin{align}
y=\hat{y}\left(r,m_{0},g_{0}\right) & =r(\cdot \mid \bx,t)\bullet l(\cdot \mid m_{0},g_{0})=\sum_{u=1}^{t}\frac{r(u\mid \bx,t)}{1+\exp(-g_{0}\left[u-m_{0}\right])}\label{eq:marginalizing_curve}
\end{align}
where $\bullet$ is a dot product, a Logistic function $l(\cdot\mid m_{0},g_{0})$
is parameterized by a growth parameter $g_{0}$ defining a slope and
the middle point of the curve $m_{0}$. The optimal parameters $g_{0}$
and $m_{0}$ will be estimated directly from the data. We illustrate
different shapes of $l$ parameterized by $g_{0}$ and $m_{0}$ in
the appendix. The Sigmoid preference has a  number of desirable properties.
As the early weights are small, less credit is given to fluctuations
at the initial stages, making it less likely for our surrogate to
be biased towards randomly well performing settings. However, as weights
monotonically increase, hyperparameters for improving performance
are preferred. As weights saturate over time, stable, high performing
configurations are preferred over short ``performance spikes'' characteristic
of unstable training. Lastly, this utility score assigns higher values
to the same performance if it is being maintained over more episodes.


\paragraph{Learning the transformation function from data.}

Different compression curves $l()$, parameterized by different choices
of $g_{0}$ and $m_{0}$ in Eq. (\ref{eq:marginalizing_curve}), may
lead to different utilities $y$ and thus affect the performance.
The optimal values of $g_{0}^{*}$ and $m_{0}^{*}$ are unknown in
advance. Therefore, we propose to learn these values $g_{0}^{*}$
and $m_{0}^{*}$ directly from the data. Our intuition is that the
`optimal' compression curve $l(m_{0}^{*},g_{0}^{*})$ will lead to
better fitting for the GP. This better GP surrogate model, thus, will
result in better prediction as well as optimization performance.
We parameterize the GP log marginal likelihood $L$ \cite{Rasmussen_2006gaussian}
as the function of $m_{0}$ and $g_{0}$:
\begin{align}
L(m_{0},g_{0})= & \frac{1}{2}\hat{\by}^{T}\left(\bK+\sigma_{y}^{2}\idenmat\right)^{-1}\hat{\by}-\frac{1}{2}\ln\left|\bK+\sigma_{y}^{2}\idenmat\right|+\textrm{const}\label{eq:MarginalLLK}
\end{align}
where $\sigma_{y}^{2}$ is the output noise variance, $\hat{\by}$
is the function of $m_0$ and $g_{0}$ defined in Eq. (\ref{eq:marginalizing_curve}).
We optimize $m_{0}$ and $g_{0}$ (jointly with other GP hyperparameters)
using multi-start gradient descent. We derive the derivative $\frac{\partial L}{\partial m_{0}}=\frac{\partial L}{\partial\hat{y}}\frac{\partial\hat{y}}{\partial m_{0}}$
and $\frac{\partial L}{\partial g_{0}}=\frac{\partial L}{\partial\hat{y}}\frac{\partial\hat{y}}{\partial g_{0}}$
which can be computed analytically as:\vspace{-15pt}

\begin{center}
\begin{minipage}[t]{0.29\columnwidth}%
\begin{align*}
\frac{\partial L}{\partial\hat{y}} & =\left(\bK+\sigma_{y}^{2}\idenmat_{N}\right)^{-1}\hat{y};
\end{align*}
%
\end{minipage}\hfill{}%
\begin{minipage}[t]{0.35\columnwidth}%
\begin{align*}
\frac{\partial\hat{y}}{\partial m_{0}} & =\frac{-g_{0}\times\exp(-g_{0}\left[u-m_{0}\right])}{\left[1+\exp(-g_{0}\left[u-m_{0}\right])\right]^{2}};
\end{align*}
%
\end{minipage}\hfill{}%
\begin{minipage}[t]{0.35\columnwidth}%
\begin{align*}
\frac{\partial\hat{y}}{\partial g_{0}} & =\frac{-m_{0}\times\exp(-g_{0}\left[u-m_{0}\right])}{\left[1+\exp(-g_{0}\left[u-m_{0}\right])\right]^{2}}.
\end{align*}
%
\end{minipage}
\par\end{center}


The estimated compression curves are illustrated in Right Fig. \ref{fig:VirtualObs_LogisticScore-3}
and in Sec. \ref{subsec:Model--illustration}. 

 

\subsection{Augmenting the training data\label{subsec:Augmentation-with-intermediate}}

When evaluating a parameter $\bx$ over $t$ iterations, we obtain
not only a final score but also all reward sequences $r(t' \mid \bx,t),\forall t'=1,...,t$.
The auxiliary information from the curve can be useful 
for BO. Therefore, we propose to augment the information from the
curve into the sample set of our GP model. 

%\paragraph{Ill-conditioned issue with augmenting a full curve.}
A na\"ive approach for augmentation is to add a full curve of points
$\{[\bx,j],y_{j}\}_{j=1}^{t}$ where $y_{j}$ is computed  using
Eq. (\ref{eq:marginalizing_curve}). However, this approach can be redundant and may impose
serious issues in the conditioning of the GP covariance matrix. As
we cluster more evaluations closely, the conditioning of the GP covariance
degrades further, as discussed in \cite{mcleod2018optimization}.
This conditioning issue is especially serious in our noisy DRL settings.
\begin{figure}
\begin{centering}
\vspace{-0pt}
\par\end{centering}
\begin{centering}
\par\end{centering}
\begin{centering}
\includegraphics[width=0.5\columnwidth]{fig/GP/2_GP2d}\includegraphics[width=0.5\columnwidth]{fig/GP/2_GP2d_fullM}
\par\end{centering}
\begin{centering}
\vspace{-5pt}
\caption{GP with different settings. Left: our augmentation. Right: using
a full curve.  If we add too much observations, the GP covariance
matrix becomes ill-conditioned. In Right, the GP is not well estimated
that the GP mean is significantly small and large $\left[-400,240\right]$
although the output is standardized $\mathcal{N}(0,1)$. All x-axis
are over $x$, a hyperparameter to be tuned. \label{fig:GP_Example}}
\par\end{centering}
\vspace{-10pt}
\end{figure}
\begin{wrapfigure}{o}{0.47\columnwidth}%
\begin{centering}
\vspace{-10pt}
\includegraphics[width=0.47\columnwidth]{fig/cond_number_3d}
\par\end{centering}
\begin{centering}
\vspace{-6pt}
\caption{The condition number of GP covariance matrix goes badly if we add
the whole curve of points into a GP. The large condition number measures
the nearness to singularity. \label{fig:Condition-number-of-1}}
\par\end{centering}
\vspace{-20pt}
\end{wrapfigure}We highlight this effect on GP estimation in Fig. \ref{fig:GP_Example}
wherein the GP mean estimation goes off significantly large and small
due to the undesirable effect of the GP covariance condition number when the \emph{natural log} of condition number goes above $25$ (see Fig. \ref{fig:Condition-number-of-1}) if we augment the whole curve. 

\paragraph{Selecting subset of points from the curve.}
 Different solutions, such as the addition of artificial noise or altering the kernel's length-scales, have been proposed. We select to use the active learning approach \cite{osborne2012active,gal2017deep} as sampled data points are expected to contain a lot of redundant information. As a consequence, the loss of information from sub-sampling the data should be minimal and information-eroding modification of the kernel matrix
 itself can be avoided. As a side benefit, the reduced number of sampled points speeds up inference in our GP models.

%We can mitigate such conditioning issue by selecting a subset of points from the curve whilst discouraging the addition of similar points. 

Particularly, we select 
samples at the maximum of the GP predictive uncertainty.  Formally,
we sequentially select a set $Z=[z_{1},...z_{M}]$, $z_{m}=\left[\bx,t_{m}\right]$,
by varying $t_{m}$ while keeping $\bx$ fixed as
\begin{align}
z_{m}= & \arg\max_{\forall t'\le t}\thinspace\sigma([\bx,t']\mid D'),\forall m\le M\,\,\,\,\textrm{s.t}.\,\,\,\,\textrm{ln}\,\textrm{of\,cond}(K)\le\delta\label{eq:Augmentation}
\end{align}
where $D'=D\cup\{z_{j}=[\bx,t_{j}]\}_{j=1}^{m-1}$. This sub-optimisation
problem is done in a one-dimensional space of $t'\in\{T_{\textrm{min}},...,t\}$,
thus it is \emph{cheap} to optimize using (multi-start) gradient descent (the
derivative of GP predictive variance is available \cite{Rasmussen_2006gaussian}). Alternatively, the fixed-size grid can be considered, but it may cause conditioning issues when a point in a fixed grid $\left[\bx,t_{\textrm{grid}}\right]$ is placed near
another existing point $\left[\bx',t_{\textrm{grid}}\right]$, i.e.,
$||\bx-\bx'||_{2}\le\epsilon$ for a very small value of $\epsilon$.

These generated points $Z$ are used to calculate the output $r(z_{m})$
and augmented into the observation set $\left(X,Y\right)$ for fitting
the GP. The number of samples $M$ is adaptively chosen such
that the natural log of the condition number of the covariance matrix
is less than a threshold. This is  to ensure that the GP covariance
matrix condition number behaves well by reducing the number of unnecessary
points added to the GP at later stages.  We compute the utility score
$y_{m}$ given $z_{m}$ for each augmented point using Eq. (\ref{eq:marginalizing_curve}).
In addition, we can estimate the running time $c_{m}$ using the predictive
mean $\mu_{c}(z_{m})$.  We illustrate the augmented observations
and estimated scores in Fig. \ref{fig:VirtualObs_LogisticScore-3}.

% \begin{algorithm}
% \caption{Bayesian Optimization with Iterative Learning (BOIL)\label{alg:BO_DRL}}
% \begin{algor}
% \item [{{*}}] \textbf{Input}: \#iter $N$, initial data $D_0$, $\bz=\left[\bx,t\right].$
% \textbf{Output}: optimal $\bx^*$ and $y^*=\max_{\forall y\in D_{N}}y$
% \end{algor}
% \begin{algor}[1]
% \item [{for}] $n=1....N$
% \item [{{*}}] Fit two GPs to calculate $\mu_{f}(),\sigma_{f}()$ and $\mu_{c}()$
% from Eqs. (\ref{eq:mu_f},\ref{eq:sigma_f},\ref{eq:mu_c}).
% \item [{{*}}] Select $\bz_{n}=\arg\max_{\bx,t}\alpha(\bx,t)/\mu_{c}(\bx,t)$
% and observe a curve $r$ and a cost $c$ from $f(\bz_{n})$
% \item [{{*}}] Compressing the learning curve $r(\bz_{n})$ into numeric
% score using Eq. (\ref{eq:marginalizing_curve}).
% \item [{{*}}] Sample augmented points $\bz_{n,m},y_{n,m},c_{n,m},\forall m\le M$
% given the curve and $D_{n}$ in Eq. (\ref{eq:Augmentation})
% \item [{{*}}] Augment the data into $D_{n}$ and estimate Logistic curve
% hyperparameters $m_{0}$ and $g_{0}$.
% \item [{endfor}]
% \end{algor}
% \end{algorithm}



\begin{algorithm}
\caption{Bayesian Optimization with Iterative Learning (BOIL)\label{alg:BO_DRL}}

\begin{algor}
\item [{{*}}] \textbf{Input}: \#iter $N$, initial data $D_{0}$, $\bz=\left[\bx,t\right]$.
\textbf{Output}: optimal $\bx^{*}$ and $y^{*}=\max_{\forall y\in D_{N}}y$
\end{algor}
\begin{algor}[1]
\item [{for}] $n=1....N$
\item [{{*}}] Fit two GPs to calculate $\mu_{f}(),\sigma_{f}()$ and $\mu_{c}()$
from Eqs. (\ref{eq:mu_f},\ref{eq:sigma_f},\ref{eq:mu_c}).
\item [{{*}}] Select $\bz_{n}=\arg\max_{\bx,t}\alpha(\bx,t)/\mu_{c}(\bx,t)$
and observe a curve $r$ and a cost $c$ from $f(\bz_{n})$
\item [{{*}}] Compressing the learning curve $r(\bz_{n})$ into numeric
score using Eq. (\ref{eq:marginalizing_curve}).
\item [{{*}}] Sample augmented points $\bz_{n,m},y_{n,m},c_{n,m},\forall m\le M$
given the curve and $D_{n}$ in Eq. (\ref{eq:Augmentation})
\item [{{*}}] Augment the data into $D_{n}$ and estimate Logistic curve
hyperparameters $m_{0}$ and $g_{0}$.
\item [{endfor}]~
\end{algor}
\end{algorithm}

 We summarize the overall algorithm in Alg. \ref{alg:BO_DRL}. To enforce non-negativity and numerical stability, we make use of the transformations $\alpha\leftarrow\log\left[1+\exp(\alpha)\right]$
and $\mu_{c}\leftarrow\log\left[1+\exp(\mu_{c})\right]$.
%  in the utility $\alpha$ and cost $\mu_{c}$
